Real-time Noise Source Estimation of a Camera System from an Image and Metadata

Autonomous machines must self-maintain proper functionality to ensure the safety of humans and themselves. This pertains particularly to its cameras as predominant sensors to perceive the environment and support actions. A fundamental camera problem addressed in this study is noise. Solutions often focus on denoising images a posteriori, that is, fighting symptoms rather than root causes. However, tackling root causes requires identifying the noise sources, considering the limitations of mobile platforms. This work investigates a real-time, memory-efficient and reliable noise source estimator that combines data- and physically-based models. To this end, a DNN that examines an image with camera metadata for major camera noise sources is built and trained. In addition, it quantifies unexpected factors that impact image noise or metadata. This study investigates seven different estimators on six datasets that include synthetic noise, real-world noise from two camera systems, and real field campaigns. For these, only the model with most metadata is capable to accurately and robustly quantify all individual noise contributions. This method outperforms total image noise estimators and can be plug-and-play deployed. It also serves as a basis to include more advanced noise sources, or as part of an automatic countermeasure feedback-loop to approach fully reliable machines.

==> figICX285Cellar+doubleThermalNoise.tex <==
\begin{figure*}[t]
    \tikzsetnextfilename{FigICX285CellarPlus}
    \begingroup
        \pgfplotsset{every axis/.style={scale=0.55}}
        \pgfplotsset{cycle list/Set1, cycle multiindex* list={
                mark list*\nextlist
                Set1\nextlist
            }
        }
        \input{plotICX285Cellar+doubleThermalNoise.tex}
    \endgroup
    \caption{\emph{ICX285 sensor, Cellar + doubleThermalNoise.}
    Test
    }
    %\vspace{-0.5ex}
    \label{fig:ICX285Cellar+doubleThermalNoise}
\end{figure*}


==> figICX285Cellar.tex <==
\begin{figure*}[t]
    \tikzsetnextfilename{FigICX285Cellar}
    \begingroup
        \pgfplotsset{every axis/.style={scale=0.52}}
        \pgfplotsset{cycle list/Set1, cycle multiindex* list={
                mark list*\nextlist
                Set1\nextlist
            }
        }
        \input{plotICX285Cellar.tex}
    \endgroup
    \caption{\emph{Qualitative results}
    Test
    }
    %\vspace{-0.5ex}
    \label{fig:ICX285Cellar}
\end{figure*}


==> figICX285CellarCorrupted.tex <==
\begin{figure*}[t]
    \tikzsetnextfilename{FigICX285CellarCorrupted}
    \begingroup
        \pgfplotsset{every axis/.style={scale=0.52}}
        \input{plotICX285CellarCorrupted.tex}
    \endgroup
    %\vspace{-1.5ex}
    \caption{\emph{Noise source estimation on unexpected noise (dataset: \cellar{}, camera: \ICX285{})}. 
    Top row: Image noise increased by random Gaussian noise $\mathcal{N}(\mu = 0, \sigma = \SI{5}{\DN})$. 
    Bottom row: Model noise increased by doubling camera parameter \emph{thermal white noise}.
    Compare to top row from \cref{fig:ICX285CellarParkingLotNoiseSources}.
    }
    %\vspace{-1.5ex}
    \label{fig:ICX285CellarCorrupted}
\end{figure*}


==> tabCameraParameterConfig.tex <==
\begin{table}[t]
\caption{\emph{Configuration of variable camera metadata} used for noise source estimation (including variable metadata not used at inference time).
\label{tab:cameraConfiguration}
}
        \begin{tabular}{ll}
            \toprule
            Camera Parameter & Value \\
            \midrule
            \textbf{Sony ICX 285} & \\
            Charge Node Reference Voltage & $\SI{5}{\volt}$ \\
            Dark Signal Figure of Merit & \num{0.008891} \\
            Full Well Capacity & \num{14000} \\
            Pixel Clock Rate & $ 28.64 \times 10^6 \si{\hertz}$ \\
            Sense Node Gain & $ 5 \times 10^{-6} \si{\hertz}$ \\
            Sensor Pixel Size & $\SI{6.45}{\micro\meter}$\\
            Sensor Type & CCD \\
            Thermal White Noise & $ 30.8 \times 10^{-9} \si{\volt\per\hertz\tothe{0.5}}$ \\
            [2ex]
            \textbf{EV2 EV76C661} & \\
            Charge Node Reference Voltage & $\SI{3.3}{\volt}$ \\
            Dark Signal Figure of Merit & \num{0.956918} \\
            Full Well Capacity & \num{8400} \\
            Pixel Clock Rate & $90 \times 10^6 \si{\hertz}$ \\
            Sense Node Gain & $ 5 \times 10^{-6} \si{\volt\per\electron}$ \\
            Sensor Pixel Size & $\SI{5.3}{\micro\meter}$\\
            Sensor Type & CMOS \\
            Thermal White Noise & $ 59 \times 10^{-9} \si{\volt\per\hertz\tothe{0.5}}$ \\
            \bottomrule%
        \end{tabular}%
\end{table} 
%\vspace{-3pt}

==> tabSotaComparisonNoiseResults.tex <==
\begin{table}[h]
    \caption{\emph{Total noise estimation comparing three state-of-the-art reference methods to our best noise source estimator \fullMetadataTitle{} on synthetically corrupted (\emph{Random}) and real-world noised (\ICX285{} and \EV76C661{}) datasets.} The best results per camera and method are highlighted in bold. Note that the uncorrupted KITTI dataset may already contain considerable image noise (cf. \cref{fig:datasetsGTNoise}) and that the results should therefore be interpreted with caution.\label{tab:sotaNoiseEstimationResults}}
    %\centering
    \begin{adjustbox}{max width=0.99\linewidth}
        \setlength{\tabcolsep}{4pt}
        \begin{tabular}{llcccccccccccc}
            \toprule
            &&\multicolumn{3}{c}{KITTI}&\multicolumn{3}{c}{Sim}&\multicolumn{3}{c}{Tampere 17} &\multicolumn{3}{c}{Udacity}%
            \\
            \cmidrule(r){3-5}\cmidrule(r){6-8}\cmidrule(r){9-11}\cmidrule(r){12-14}
            & & Bias & Std & RMS & Bias & Std & RMS & Bias & Std & RMS & Bias & Std & RMS \\
            \midrule
            \parbox[t]{3.0mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Random}}}
                &B+F%   
                        & \textbf{0.00} & 2.09 & 2.09 %
                        & 2.51 & 3.00 & 3.91 %
                        & 2.22 & 4.19 & 4.74 %
                        & 1.09 & 2.19 & 2.44\\
                &\baselineTitle%     
                        & 0.03 & \textbf{0.34} & \textbf{0.35} %
                        & \textbf{0.07} & \textbf{0.23} & \textbf{0.23} %
                        & 0.21 & 0.44 & 0.49 %
                        & \textbf{0.14} & \textbf{0.42} & \textbf{0.45}\\
                &PCA%     
                        & 1.74 & 1.36 & 2.21 %
                        & 0.75 & 1.07 & 1.30 %
                        & 2.81 & 3.04 & 4.14 %
                        & 0.70 & 0.93 & 1.17\\
                &\PGETitle%     
                        & 4.00 & 4.80 & 6.24 %
                        & 3.23 & 4.36 & 5.43 %
                        & 3.15 & 3.34 & 4.59 %
                        & 3.04 & 3.70 & 4.79\\
                &\fullMetadataTitle%     
                        & 0.03 & \textbf{0.34} & \textbf{0.35} %
                        & 0.16 & 0.29 & 0.33 %
                        & \textbf{0.05} & \textbf{0.43} & \textbf{0.43} %
                        & \textbf{0.14} & \textbf{0.42} & \textbf{0.45}\\
            [1.9ex]%
            \parbox[t]{3.0mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{ICX285}}}
                &B+F%     
                        & 0.30 & 0.64 & 0.71 %
                        & 3.12 & 1.60 & 3.51 %
                        & 2.71 & 3.54 & 4.46 %
                        & 0.33 & 0.58 & 0.66\\
                &\baselineTitle%     
                        & \textbf{0.09} & \textbf{0.32} & \textbf{0.33} %
                        & 0.17 & 0.28 & 0.33 %
                        & 0.37 & 0.40 & 0.55 %
                        & \textbf{0.01} & 0.53 & 0.53\\
                &PCA%     
                        & 0.53 & 0.68 & 0.86 %
                        & 1.11 & 0.82 & 1.38 %
                        & 3.07 & 2.77 & 4.14 %
                        & 0.14 & 0.63 & 0.64\\
                &\PGETitle%     
                        & 3.06 & 1.50 & 3.41 %
                        & 3.11 & 1.26 & 3.35 %
                        & 2.74 & 1.71 & 3.23 %
                        & 3.00 & 1.48 & 3.35\\
                &\fullMetadataTitle%     
                        & 0.45 & 0.76 & 0.89 %
                        & \textbf{0.04} & \textbf{0.19} & \textbf{0.20} %
                        & \textbf{0.13} & \textbf{0.36} & \textbf{0.38} %
                        & 0.25 & \textbf{0.30} & \textbf{0.39}\\
            [1.9ex]%
            \parbox[t]{3.0mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{EV76C661}}}
                &B+F%     
                        & 0.38 & 0.72 & 0.81 %
                        & 2.90 & 1.52 & 3.28 %
                        & 2.51 & 3.40 & 4.23 %
                        & 0.11 & 0.39 & 0.40\\
                &\baselineTitle%     
                        & \textbf{0.05} & \textbf{0.23} & \textbf{0.23} %
                        & 0.14 & \textbf{0.22} & \textbf{0.26} %
                        & 0.31 & \textbf{0.37} & 0.48 %
                        & 0.10 & 0.42 & 0.43\\
                &PCA%     
                        & 1.70 & 0.93 & 1.94 %
                        & 0.89 & 0.76 & 1.17 %
                        & 2.76 & 2.66 & 3.83 %
                        & \textbf{0.04} & 0.30 & \textbf{0.30}\\
                &\PGETitle%     
                        & 3.70 & 1.25 & 3.90 %
                        & 3.65 & 1.13 & 3.82 %
                        & 3.39 & 1.64 & 3.77 %
                        & 3.41 & 0.98 & 3.55\\
                &\fullMetadataTitle%     
                        & 0.21 & 1.03 & 1.05 %
                        & \textbf{0.02} & 0.26 & \textbf{0.26} %
                        & \textbf{0.13} & 0.39 & \textbf{0.41} %
                        & 0.28 & \textbf{0.29} & 0.40\\
            \bottomrule
        \end{tabular}%
    \end{adjustbox}
\end{table} 


==> tikz/dummy.tex <==
 
